Programmable In-Network Security for Context-aware BYOD Policies

Bring Your Own Device (BYOD) has become the new norm in enterprise networks, but BYOD security remains a top concern. Context-aware security, which enforces access control based on dynamic runtime context, holds much promise. Recent work has developed SDN solutions to collect device context for network-wide access control in a central controller. However, the central controller poses a bottleneck that can become an attack target, and processing context changes at remote software has low agility. We present a new paradigm, programmable in-network security (Poise), which is enabled by the emergence of programmable switches. At the heart of Poise is a novel switch primitive, which can be programmed to support a wide range of context-aware policies in hardware. Users of Poise specify concise policies, and Poise compiles them into different instantiations of the security primitive in P4. Compared to centralized SDN defenses, Poise is resilient to control plane saturation attacks, and it dramatically increases defense agility.

==> Makefile <==
TARGET   = paper
TEXFILES = $(wildcard *.tex)
FIGURES  = compiler-performance traffic-overhead throughput delay memory overall traffic cpu sdn-delay sdn-throughput \
ctx-num-range ctx-num-delay ctx-num-throughput


.SUFFIXES:	.plot .eps .fig

all: $(TARGET).pdf

$(TARGET).aux: $(TEXFILES)
	pdflatex $(TARGET).tex

$(TARGET).bbl: $(TARGET).aux $(TARGET).bib
	bibtex $(TARGET)

$(TARGET).pdf: $(TEXFILES) $(addprefix figures/, $(addsuffix .pdf, $(FIGURES))) $(TARGET).bbl
	pdflatex $(TARGET).tex
	pdflatex $(TARGET).tex
	gs -q -dBATCH -dNOPAUSE -dSAFER -sDEVICE=pdfwrite -sOutputFile=$(TARGET)_embed.pdf -dPDFSETTINGS=/prepress $(TARGET).pdf
	mv $(TARGET)_embed.pdf $(TARGET).pdf

figures/%.pdf: figures/%.plot
	gnuplot $<

diff: diff.pdf

diff.tex: $(TEXFILES) texdiff $(TARGET).bbl
	./texdiff submission/$(TARGET).tex $(TARGET).tex >diff.tex

diff.pdf: diff.tex $(addprefix figures/, $(addsuffix .pdf, $(FIGURES)))
	pdflatex diff.tex
	bibtex ${TARGET}
	pdflatex diff.tex
	rm -f diff.tex

texdiff: figures/texdiff.cc
	g++ $< -o $@

submission/$(TARGET).tex:
	@echo Please check out a previous version of the paper, compile it, and put it into a directory called 'submission/'!
	@false

view:: $(TARGET).pdf
	xpdf $(TARGET).pdf

clean::
	rm -fv *.dvi *.aux *.log *~ *.bbl *.blg *.toc *.ps *.pdf *.eps *.cb _diff.* *.out diff.tex diff.ps diff.pdf texdiff
	rm -fv $(addprefix figures/, $(addsuffix .pdf, $(FIGURES)))

